Causal Regularization

In application domains such as healthcare, we want accurate predictive models that are also causally interpretable. In pursuit of such models, we propose a causal regularizer to steer predictive models towards causally-interpretable solutions and theoretically study its properties. In a large-scale analysis of Electronic Health Records (EHR), our causally-regularized model outperforms its L1-regularized counterpart in causal accuracy and is competitive in predictive performance. We perform non-linear causality analysis by causally regularizing a special neural network architecture. We also show that the proposed causal regularizer can be used together with neural representation learning algorithms to yield up to 20% improvement over multilayer perceptron in detecting multivariate causation, a situation common in healthcare, where many causal factors should occur simultaneously to have an effect on the target variable.

==> discussion.tex <==
\section{WHY DOES CAUSAL REGULARIZATION HELP PREDICTION?}
Figures~\ref{fig:auc_sutter}~and~\ref{fig:auc_mimic} show that \emph{causal regularization can improve prediction accuracy}. This might appear counterintuitive: after all, a prediction algorithm is designed to extract from the data all the information relevant to the prediction task. However, choosing causal predictors makes the prediction \emph{invariant under intervention}, which is crucial if the statistics of the data are prone to change with time due to external factors.

\begin{figure}
\centering
\includegraphics{Figs/smoking.png}
\caption{Fisher's take on smoking and cancer. (a) A controversial model in which genetics predispose people both to smoking and dying of lung cancer. (b) The widely accepted model in which smoking causes cancer.}
\label{fig:cancer_cigarettes}
\end{figure}

To illustrate this idea, consider Ronald Fisher's controversial claim that cigarettes do not cause cancer --- but genetics do~\citep{fisher58}. In this model, shown in Fig.~\ref{fig:cancer_cigarettes}(a), there is a genetic predisposition in some people to smoke, and the same genes responsible for the predisposition cause lung cancer; however, smoking itself does not cause cancer. 

Now, imagine one trains a predictor of lung cancer in Fisher's world. The model might learn that if you smoke, you are likely to die of lung cancer, and if you do not, the likelihood is negligible. However, this prediction is not robust with respect to external interventions. For example, the government could raise the cigarette tax tenfold and thus decrease the number of smokers to near zero. The predictor would then expect barely anyone to die of lung cancer, but this prediction would be wrong, as people's genetics remained unchanged.

To the contrary, imagine that smoking does indeed cause lung cancer --- Fig.~\ref{fig:cancer_cigarettes}(b). The predictor  would remain correct after the introduction of the tax: people who smoke less die of cancer less.

We claim that this invariance of causal prediction under intervention is what makes our causal regularizer robust on test data. In domains such as medicine, intervention on the predictive factors is very common. For example, improvements in medical technology can prevent previously unavoidable conditions, government policy can encourage or discourage health-related behaviors, and environmental changes influence our bodies.

We further note that in specific statistical scenarios (such as semi-supervised learning, transfer learning, etc) learning only the causal predictors might be preferable. These situations are enumerated and explained in detail by~\citet{Storkey2009}~and~\citet{Janzing2012}. We do not repeat the discussion here, as it is mostly applicable beyond simple regression scenarios.

%@article{fisher1958,
%  title={Cigarettes, cancer, and statistics},
%  author={Fisher, Ronald},
%  journal={The Centennial Review of Arts \& Science},
%  volume={2},
%  pages={151--166},
%  year={1958},
%  publisher={JSTOR}
%}
%
%@inproceedings{Janzing2012,
%  title={On causal and anticausal learning},
%  author={Janzing, Dominik and Peters, Jonas and Sgouritsa, Eleni and Zhang, Kun and Mooij, Joris M and Sch{\"o}lkopf, Bernhard},
%  booktitle={Proceedings of the 29th International Conference on Machine Learning (ICML-12)},
%  pages={1255--1262},
%  year={2012}
%}
%
%@article{Storkey2009,
%  title={When training and test sets are different: characterizing learning transfer},
%  author={Storkey, Amos},
%  journal={Dataset shift in machine learning},
%  pages={3--28},
%  year={2009},
%  publisher={Cambridge, MA: MIT Press}
%}

==> setting.tex <==
\usepackage{bm,amsmath,amssymb}
\usepackage{paralist}
\usepackage{graphicx}
\usepackage{fullpage}
\usepackage{hyperref}
\usepackage{longtable,lscape}
\usepackage[normalem]{ulem}
\usepackage{booktabs}
\usepackage{xspace}
\usepackage{tcolorbox}
\tcbuselibrary{skins,breakable}
\RequirePackage{color}
\newtheorem{theorem}{Theorem}
%\newtheorem*{theorem*}{Theorem}
% \newtheorem*{theorem*}{Theorem}
\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
\hypersetup{ % play with the different link colors here
    colorlinks,
    citecolor=mydarkblue,
    filecolor=mydarkblue,
    linkcolor=mydarkblue,
    urlcolor=mydarkblue % set to black to prevent printing blue links
}
% \usepackage{array}
% \newcolumntype{L3}{>{\centering\arraybackslash}m{3cm}}
% \newcolumntype{L8}{>{\centering\arraybackslash}m{8cm}}
\usepackage{array}
\usepackage{sidecap}
\sidecaptionvpos{figure}{c}
\usepackage{natbib}
\usepackage{subcaption}
% \renewcommand{\arraystretch}{1.3}
\renewcommand{\arraystretch}{1.2}

% \usepackage{wrapfig}
% \usepackage{floatrow}
% \newfloatcommand{capbtabbox}{table}[][\FBwidth]
% \floatsetup[table]{capposition=top}
\usepackage{url}
\usepackage{newfloat}
\usepackage{multirow}
\usepackage{balance}
\DeclareCaptionType{Algorithm}
\newcommand{\tbedit}[1]{\textcolor{magenta}{\emph{[TB: #1]}}}
\newcommand{\jsedit}[1]{\textcolor{olive}{\emph{[JS: #1]}}}
\newcommand{\kcedit}[1]{\textcolor{blue}{\emph{[KC: #1]}}}
\newcommand{\feedit}[1]{\textcolor{green}{\emph{[FE: #1]}}}
\newcommand{\blue}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\red}[1]{\textcolor{red}{\textbf{#1}}}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
% \usepackage[top=1in, bottom=1.25in, left=1in, right=1in]{geometry}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{bm}
\usepackage{enumitem}

\newenvironment{block}[1]{%
    \tcolorbox[beamer,%
    noparskip,breakable,
    colback=LightBlue,colframe=DarkBlue,%
    colbacklower=DarkBlue!75!LightBlue,%
    title=#1]}%
    {\endtcolorbox}

\newenvironment{block2}[1]{%
    \tcolorbox[beamer,%
    noparskip,breakable,
    colback=Azure,colframe=RoyalBlue,%
    colbacklower=LightSteelBlue!75!Azure,%
    title=#1]}%
    {\endtcolorbox}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}

\newcommand{\cs}{X}
\newcommand{\ef}{Y}
